Provable Filter Pruning for Efficient Neural Networks

We present a provable, sampling-based approach for generating compact Convolutional Neural Networks (CNNs) by identifying and removing redundant filters from an over-parameterized network. Our algorithm uses a small batch of input data points to assign a saliency score to each filter and constructs an importance sampling distribution where filters that highly affect the output are sampled with correspondingly high probability. In contrast to existing filter pruning approaches, our method is simultaneously data-informed, exhibits provable guarantees on the size and performance of the pruned network, and is widely applicable to varying network architectures and data sets. Our analytical bounds bridge the notions of compressibility and importance of network structures, which gives rise to a fully-automated procedure for identifying and preserving filters in layers that are essential to the network's performance. Our experimental evaluations on popular architectures and data sets show that our algorithm consistently generates sparser and more efficient models than those constructed by existing filter pruning approaches.

==> notes/propagated.tex <==
\section{Propagated sensitivity}
The idea is to take a weighted sum of sensitivities during a backwards pass. We derive the operations for linear layers and convolutional layers below. 

\subsection{Linear layer}
For layer $\ell$, let $z^\ell = W^\ell a^{\ell - 1}$, where $a^{\ell -1 } \in \Reals^{\eta^{\ell -1}}$, $z^\ell \in \Reals^{\eta^\ell}$, and $W^\ell \in \Reals^{\eta^{\ell} \times \eta^{\ell-1}}$. We define the edge sensitivity $g_{ij}$ for an input $x$ as 
\begin{equation}
\label{eq:g}
g_{ij}^{\ell} = \frac{w_{ij}^{\ell} a_j^{\ell-1}}{\sum_{k \in [\eta^{\ell-1}]} w_{ik}^{\ell} a_k^{\ell-1}} = \frac{w_{ij}^{\ell} a_j^{\ell-1}}{z_i^\ell}.    
\end{equation}

We are sloppy and dropping the $x$ for now from notation to avoid clutter. We let the (normalized) sensitivity of neuron $i$, $i \in [\eta^\ell]$, in layer $\ell$ be denoted by $\beta^\ell_i$. We let the (unnormalized) sensitivity $\alpha^{\ell - 1}_j$ of neuron $j$, $j \in [\eta^{\ell -1}]$, in layer $\ell - 1$ be defined as 
\begin{equation}
\label{eq:alpha}
\alpha^{\ell - 1}_j = \sum_{i \in [\eta^\ell]} \beta^\ell_i g_{ij}^{\ell}.
\end{equation}

We would like to find an efficient, i.e., tensorized, way to compute $\alpha^{\ell -1} \in \Reals^{\eta^{\ell-1}}$. Plugging \eqref{eq:g} into \eqref{eq:alpha}, we obtain
\begin{align*}
\alpha^{\ell -1}_j
&= \sum_{i \in [\eta^\ell]} \beta^\ell_i \frac{w_{ij}^{\ell} a_j^{\ell-1}}{z_i^\ell} \\
&= a_j^{\ell - 1} \sum_{i \in [\eta^\ell]} \frac{\beta_i^{\ell}}{z_i^\ell} w_{ij}^\ell \\
&= a_j^{\ell - 1} \dotp{\beta^\ell \oslash z^\ell}{ w_{j}^\ell},
\end{align*}
where $w_j^\ell$ denotes the $j$th column of $W^\ell$. We can rewrite this in matrix notation as
$$
\alpha^{\ell-1} = a^{\ell - 1} \odot \left((W^\ell)^T (\beta^\ell \oslash z^\ell)\right).
$$

We also need to pass on the (normalized) sensitivity of neurons $\beta^{l - 1}$, which we simply get as 
$$
\beta^{l - 1} = \frac{1}{\sum_j \alpha_j^{\ell -1}} \alpha^{\ell - 1}.
$$
Note that there is a nice analogy to the derivative $\frac{\partial L}{\partial a^{\ell -1}}$, which is passed on the previous layer during the backwards pass in a network: 

$$
\begin{array}{l| c }
& \text{input}  \\ \hline 
& \\
\text{derivative} & \nicefrac{\partial L}{\partial a^{\ell -1}}  =  (W^\ell)^T \nicefrac{\partial L}{\partial z^\ell} \\
& \\
\text{sensitivity} &  \alpha^{\ell-1} \oslash a^{\ell - 1}  = (W^\ell)^T (\beta^\ell \oslash z^\ell) \\
& \\
\end{array}
$$

\subsection{Convolutional layer}
This operation is bit trickier. Again, for layer $\ell$, let $z^\ell = W^\ell * a^{\ell - 1}$, where $a^{\ell -1 } \in \Reals^{s_1^{\ell - 1} \times s_2^{\ell - 1} \times c^{\ell -1}}$, $z^\ell \in \Reals^{s_1^{\ell} \times s_2^{\ell}}$, and $W^\ell \in \Reals^{\kappa_1^\ell \times \kappa_2^\ell \times c^{\ell-1}}$ (only one output filter for simplicity). We define the edge sensitivity $e_{ij}$, $i \in [s_1^{\ell}] \times [s_2^{\ell}]$, $j \in [\kappa_1^\ell] \times [\kappa_2^\ell] \times [c^{\ell-1}]$ for an input $x$ as 
\begin{equation}
\label{eq:econv}
e_{ij}^{\ell} = \frac{w_{j}^{\ell} a_{m_i(j)}^{\ell-1}}{\sum_{k} w_{k}^{\ell} a_{m_i(k)}^{\ell-1}} = \frac{w_{j}^{\ell} a_{m_i(j)}^{\ell-1}}{z^\ell_i},
\end{equation}
where $m_i(j) \in [s_1^{\ell - 1}] \times [s_2^{\ell - 1}] \times [c^{\ell -1}]$ denotes the mapping from weight index $j$ to the corresponding pixel index for patch $i$. Further, let $\beta_i^\ell$ denote the normalized sensitivity of patch/pixel $i$ in layer $\ell$. We then define the (unnormalized) weighted sensitivity of weight $j$ in layer $\ell$ as 
\begin{equation}
\label{eq:gconv}
    g_j^\ell = \sum_i \beta_i^\ell e_{ij}^\ell.
\end{equation}
Plugging \eqref{eq:econv} into \eqref{eq:gconv} we obtain 
\begin{align*}
g_j^\ell
&= \sum_i \beta_i^\ell \frac{w_{j}^{\ell} a_{m_i(j)}^{\ell-1}}{z^\ell_i} \\
&= w_j^\ell \sum_i \frac{\beta_i^\ell}{z^\ell_i} a_{m_i(j)}, 
\end{align*}
which we can conveniently rewrite as a convolutional operation as follows
$$
g^\ell = W^\ell \odot \left( (\beta_\ell \oslash z^\ell) * rot(a^{\ell-1}) \right).
$$
$rot(M)$ hereby denotes a $180^\circ$ rotation of some matrix $M$. This gives us the sensitivity of individual weights. We also require $\beta^{\ell-1}$ to pass it on to the previous layer. To this end, let $\alpha_k^{\ell - 1}$, $k \in [s_1^{\ell - 1}] \times [s_2^{\ell - 1}] \times [c^{\ell -1}]$, denote the (unnormalized) sensitivity of pixel $k$ in layer $\ell - 1$, which is defined as 
\begin{equation}
\label{eq:alphaconv}
\alpha_k^{\ell - 1} = \sum_i \beta_i^\ell e^\ell_{i, m^{-1}_i(k)}.
\end{equation}
Again, plugging \eqref{eq:econv} into \eqref{eq:alphaconv} we obtain
\begin{align*}
\alpha_k^{\ell - 1}
&= \sum_i \beta_i^\ell \frac{w_{m^{-1}_i(k)}^{\ell} a_{k}^{\ell-1}}{z^\ell_i} \\
&= a_k^{\ell - 1} \sum_i w^\ell_{m^{-1}_i(k)} \frac{\beta_i^\ell}{z_i^\ell}, 
\end{align*}
which can be rewritten as convolution as follows 
$$
\alpha^{\ell - 1} = a^{\ell - 1} \odot \left( rot(W^\ell) * (\beta^\ell \oslash z^\ell) \right).
$$ 
For both derivations, a picture is helpful to understand the alignment of indices. 

Again, it is interesting to draw a parallel to the derivatives computed during a backwards pass: 
$$
\begin{array}{l| c | c }
& \text{input}  & \text{weight} \\ \hline 
&& \\
\text{derivative} & \ \ \nicefrac{\partial L}{\partial a^{\ell-1}} = rot(W^\ell) * \nicefrac{\partial L}{\partial z^\ell} &   \nicefrac{\partial L}{\partial W^\ell} =   \nicefrac{\partial L}{\partial z^\ell} * rot(a^{\ell - 1}) \\
&& \\
\text{sensitivity} & \alpha^{\ell - 1} \oslash a^{\ell - 1} = rot(W^\ell) * (\beta^\ell \oslash z^\ell) &  \ \ \ g^\ell \oslash W^\ell = (\beta^\ell \oslash z^\ell) * rot(a^{\ell - 1}) \\
&& \\
\end{array}
$$

\subsection{Weighted max instead of weighted sum}
An alternative approach for sensitivity would be a weighted max instead of a weighted sum. We can derive the same result for weighted max. To derive the result, we note that we replace the convolutional operator $*$ with a maxpool operator with appropriate stride/kernel/etc... Then the exact same result applies with $* = maxpool$. 

\subsection{Negative weights}
All the results above are for positive weights only. We should think about the generalization to negative weights as well. 

==> notes/pruning-old.tex <==
\section{Sampling-based Pruning}
\label{sec:sparsification}
In this section, we introduce the core procedure of our pruning method, which is a sampling procedure over filters/neurons in each layer. To this end, let $W_j^\ell$, $j \in [\eta^\ell]$, denote the filter $j$ in the $\ell^\text{th}$ layer of a convolutional neural network, where $\eta^\ell$ denotes the number of filters in layer $\ell$. We would like to sample filters $W_j$ from the weight tensor $W^\ell = [W_1^\ell, \ldots, W^\ell_{\eta^{\ell}}]$ in layer $\ell$ according to some appropriate probability $p_j^\ell$ reflecting the salience of the corresponding feature map. We then construct a compact weight tensor $\WWHat^\ell$ from the samples, repeat the procedure for all layers, and fine-tune the network. The probability distribution $p^\ell = (p_1^\ell, \ldots, p_{\eta^\ell})$ is constructed by empirically quantifying the sensitivity of each filter $j$ in layer $\ell$ using a small batch of input data points. We proceed by introducing the sampling procedure, establishing desired properties of our sampling distribution, and introducing the notion of empirical sensitivity to define an informed sampling distribution.
% \renewcommand{\theenumi}{\Roman{enumi}}%
% \begin{enumerate}
%     \item \label{prop:unbiased}
%     the estimator should be unbiased, i.e., in expectation it should be equal to the \emph{true} output of the layer;
%     \item \label{prop:whp}
%     the estimator should work well not only in expectation, but work well with high probability (for an appropriate notion of high probability); 
%     \item \label{prop:m}
%     the estimator should be constructed using a sampling distribution that minimizes the required number of samples such that the resulting layer is significantly smaller.
% \end{enumerate}

\begin{wrapfigure}{R}{0.53\textwidth}
\begin{minipage}{0.53\textwidth}
\vspace{-5.5ex}
\begin{algorithm}[H]
\small
\caption{\textsc{PruneFilters}$(\WW^\ell, \eps, \delta, p^\ell$)}
\label{alg:sampling}
\textbf{Input:} $\WW^\ell = [\WW_1^\ell, \ldots, \WW_{\eta^\ell}^\ell]$: original filters; $\eps$: relative error; $\delta$: failure probability; $p^\ell$: sampling probabilities \\
\textbf{Output:} $\WWHat^\ell$: pruned filters
\begin{spacing}{1.1}
\begin{algorithmic}[1]
\small
\STATE $m^\ell \gets m^\ell(\eps, \delta)$ \COMMENT{set required number of samples \CB{TODO: According to Eq.?}} \label{lin:samplecomplexity}

\STATE $\mathcal{H} \gets$ distribution on $[\eta^\ell]$ s.t.\ index $j$ has probability $p_j$\label{lin:distribution}

\STATE $\WWHat^\ell \gets [0, \ldots, 0]$ \COMMENT{$\WWHat^\ell$ has same dimensions as $\WW^\ell$}

\FOR{$k \in [m^\ell]$} \label{lin:start-reweigh}
    \STATE $c(k) \gets $ random draw from $\mathcal{H}$ \label{lin:drawing}
    \STATE $\hat{W}^\ell_{c(k)} \gets \hat{W}^\ell_{c(k)} + \frac{W^\ell_{c(k)}}{m p_{c(k)}}$ \label{lin:estimator}
\ENDFOR \label{lin:end-reweigh}

% \STATE $(K_1,\ldots,K_{\eta^\ell}) \sim \text{Multinomial}\left(m^\ell, p^\ell\right)$; \COMMENT{Each $K_i$ denotes the number of times neuron $\edge$ was sampled} \label{lin:sampling}
% \FOR{$j \in [\eta^\ell]$} \label{lin:start-reweigh}
% 	\STATE $\WWHat^\ell_j \gets K_j \frac{\WW^\ell_{j}}{m^\ell \, p_j^\ell}$; \quad \COMMENT{Store the rescaled (debiased) filter of $W^\ell_j$. $K_j$ might be $0$.}
% \ENDFOR \label{lin:end-reweigh}

\STATE \textbf{return} $\WWHat = [\WWHat^\ell_1, \ldots, \WWHat^\ell_{\eta^\ell}]$;

\end{algorithmic}
\end{spacing}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\subsection{Overview}
As before, let $p^\ell$ denote the sampling distribution over filters in layer $\ell$. The sampling procedure for filters in layer $\ell$ is summarized in Algorithm~\ref{alg:sampling}. In Line~\ref{lin:samplecomplexity}, we set the required number of samples as a function of the maximum desired relative error $\eps$ and the desired maximum failure probability $\delta$. In other words, we want to sample enough times such that the compact weight tensor $\WWHat^\ell$ can approximate the \emph{true} output of subsequent layers with probability at least $1 - \delta$ up to $(1 \pm \eps)$ multiplicative error. Intuitively, we require more samples for lower $\eps$ and lower $\delta$. Moreover, as we will later see the sample complexity $m^\ell$ also drastically depends on our choice $p^\ell$. We define the distribution over filter indices $\mathcal H$ in Line~\ref{lin:distribution} and then proceed to sample $m^l$ times with replacement according to $\mathcal H$, see Lines~\ref{lin:start-reweigh}-\ref{lin:end-reweigh}. The resulting filters are rescaled by a factor that is inversely proportional to their sample probability to obtain an \emph{unbiased} estimator (see below). Note that since $m^\ell \ll \eta^\ell$, we only sample a small subset of the filters and discard the unsampled ones, which leads to a reduction in the layer's size.

%We note that in practice $m^\ell \ll \eta^\ell$, thus many filters never get sampled, i.e., $c(k) \neq j, \, \forall k \in [m^\ell]$ for some $j$, resulting in a reduced layer size.

\subsection{A Tightly-Concentrated Estimator}
In the following, we would like to better understand the properties of the pruning procedures resulting from our random sampling scheme by analyzing the effect of the pruning on the subsequent layer $\ell + 1$.
To this end, let $a^{\ell}(x)$ denote the activation of layer $\ell$ for an input point $x$ to the network and note that $a_j^{\ell}(x)$ is the $j$th feature map of layer $\ell$, which is generated by $\WW_j^\ell$. 
In addition, let $z^{\ell+1}(x)$ denote the pre-activation of layer $\ell + 1$ and for ease of presentation, assume that the layer is linear, i.e., $z^{\ell+1}(x) = W^{\ell+1} a^{\ell}(x)$, $\WW^{\ell + 1} \in \RR^{\eta^{\ell+1} \times \eta^{\ell}}$. The extension to CNNs follows directly as outlined in Appendix~\ref{sec:analysis}. We note that by replacing $\WW^\ell$ with the random quantity $\WWHat^\ell$ the pre-activation $z^{\ell+1}(x)$ is also affected. We denote the resulting random variable by $\hat z^{\ell + 1}(x)$ defined by 
$$\hat z^{\ell + 1}(x) = \sum_{k=1}^{m^\ell} \WW_{:c(k)}^{\ell + 1} \, \frac{a_{c(k)}^\ell}{m \,p_{c(k)}}, \quad \text{where} \quad c(k) \sim \mathcal H \quad \forall k,
$$
and $\WW^{\ell+1}_{:j}$ denotes the $j^\text{th}$ column of $\WW^{\ell + 1}$. Clearly, $\E_{\WWHat^\ell} [\hat z^{\ell+1}(x)] = z^{\ell+1}(x)$, i.e., $\hat z^{\ell+1}(x)$ is unbiased estimator of the pre-activation $z^{\ell+1}(x)$.

\CB{TODO for me....: Rewrite this}
In the context of Algorithm~\ref{alg:sampling} an unbiased estimator is needed to ensure good performance in expectation, however, any large deviation can substantially degrade the quality of the estimator in practice. Henceforth, we need to analyze the behavior of the estimator $\hat z^{\ell+1}$ when it deviates from its mean. Ideally, we would like the estimator to be tightly concentrated around its mean, i.e., to have low probability of deviation. As previously noted the quality of the estimator should improve when we increase the sample complexity $m^\ell$. We formalize this intuition by leveraging Bernstein's concentration inequality to calculate the number of samples required to ensure that our estimator is within $(1 \pm \eps)$ multiplicative error with probability at least $1 - \delta$. 
%We state a version of Bernstein's inequality below that enables us to compute the number of samples required to ensure that our estimator is tightly concentrated.

% \begin{theorem}[Bernstein's inequality~\cite{vershynin2016high}]
% \label{thm:bernstein}
% Let $Y_1, \ldots, Y_m$ be a sequence of $m$ i.i.d. random variables satisfying $\max_{k \in [m]} \, \abs{Y_k - \E[Y_k]} \leq R$, and let $Y = \sum_{k=1}^m Y_k$ denote their sum. Then, for every $\eps \geq 0$, $\delta \in (0, 1)$, we have that $\Pr\left(\abs{Y - \E[Y]} \geq \eps \E[Y] \right) \leq \delta$ for
% $$
% m \ge \frac{\log(2 / \delta)}{(\eps E[Y_k])^2} \left( \Var(Y_k) + \frac{2}{3} \eps \E[Y_k] R \right).
% $$
% \end{theorem}

\begin{theorem}[Bernstein's inequality~\cite{vershynin2016high}]
\label{thm:bernstein}
Let $Y_1, \ldots, Y_m$ be a sequence of $m$ i.i.d. random variables satisfying $\max_{k \in [m]} \, \abs{Y_k - \E[Y_k]} \leq R$, and let $Y = \sum_{k=1}^m Y_k$ denote their sum. Then, for every $\eps \geq 0$, $\delta \in (0, 1)$, we have that $\Pr\left(\abs{Y - \E[Y]} \geq \eps \E[Y] \right) \leq \delta$ for
$$
m \ge \frac{\log(2 / \delta)}{(\eps E[Y_k])^2} \left( \Var(Y_k) + \frac{2}{3} \eps \E[Y_k] R \right).
$$
\end{theorem}

Viewed in the context of the discussion above, we have for some $i$ the random variable $Y_{k} = W^{\ell+1}_{i c(k)} \frac{a_{c(k)}}{p_{c(k)}}$, $c(k) \sim \mathcal H$, such that $\hat z_i (x) = \sum_{k=1}^{m^\ell} Y_k$, where $\hat z_i^{\ell + 1} (x), \, i \in [\eta^{\ell+1}],$ denotes the $i^\text{th}$ entry of $\hat z^{\ell+1}(x)$.
%Viewed in the context of the reweighing procedure in Alg.~\ref{alg:prune-neurons}, we have the random variables  $Y_k = \frac{w_{ik} a}{p_k}$, 
Theorem~\ref{thm:bernstein} states that the number of samples required for a sufficiently high concentration around the mean depends on the magnitude of the centered random variables $Y_k - \E[Y_k]$, i.e., $R$, and their second moment, i.e., $\E[(Y_k - \E[Y_k])^2] = \Var(Y_k)$. By definition of $Y_k$, observe that these expressions are heavily influenced by our choice of the sampling distribution $p^\ell$.  Thus, to minimize the number of samples required to achieve high concentration\footnote{We define the minimization with respect to sample complexity from Theorem~\ref{thm:bernstein}, which serves as a sufficiently good proxy as Bernstein's inequality is optimal up to logarithmic factors~\cite{tropp2015introduction}.}  we require a judiciously defined sampling distribution that simultaneously minimizes both $R$ and $\Var(Y_k)$. For example, for $n = \eta^\ell$, the naive approach of uniform sampling, i.e., $p_j^\ell = \frac{1}{n}$ for each $j \in [n]$ also leads to an unbiased estimator, however, for uniform sampling we have $\Var(Y_k) \approx n \mu^2$ and $R \approx n \max_{k} (w_{ik} a_k)$ and so $\Var(Y_k), R \in \Omega(n)$ in the general case, leading to a linear sampling complexity $m \in \Omega(n)$ by Theorem~\ref{thm:bernstein}.

%the main crux resides within defining an appropriate sampling distribution that simultaneously minimizes the second and the infinity moment.

%Consider, for example, a uniform distribution over the parameters. The uniform distribution is known to maximize the variance, which is proportional to the sample complexity $m^\ell$ of our estimator. At this point, it should become apparent that obtaining an unbiased estimator is easy (the uniform distribution is also unbiased), but that the main crux resides within defining an appropriate sampling distribution that simultaneously minimizes the second and the infinity moment.

\subsection{An Efficient Sampling Distribution from Empirical Sensitivity}
To obtain a better sampling distribution, we leverage the notion of empirical sensitivity inspired by~\cite{blg2018}, which allows to simultaneously minimizes the variance and the magnitude of the estimator, and is efficiently computable in practice. We define the sensitivity $s_j^\ell$ of filter $j$ in $\ell$ as 
$$
a  
$$

\subsection{An Efficient Sampling Distribution from Empirical Sensitivity}
\label{sec:sensitivity}
To obtain a better sampling distribution, note that if we fix a single input $\xx \in \XX$ and neuron $i$, the distribution $p^*_k(\xx) = \frac{w_{ik}a_k(\xx)}{\sum_{k'} w_{ik'}a_{k'}(\xx)}$ simultaneously minimizes $\Var(Y_k)$ and $\max_{k} \frac{w_{ik} a_k}{p^*_k}$ such that under $p^*(\xx)$, $\Var(Y_k) \leq \E[Y_k]^2$ and $R \leq 2 \E[Y_k]$, leading to the desirable sublinear sampling complexity of $m \in \Theta( \log(2/\delta) \, \epsilon^{-2})$. While this distribution may work well in bounding the variance and magnitude for a single input point $\xx$ and neuron $i$ that are known in advance, we require our sampling procedure to work well for a multitude of input points $x \in \DD$ since we do not know the inputs that will be given to our compressed network in advance.

\paragraph{The sensitivity framework}
% The state-of-the-art coresets framework uses exact expression of $p^*_k(\xx)$ from before in constructing a more informed sampling, and alleviates the requirement that the input is known in advance by simply taking the supremum of $p_k(\xx)$ over all the input points in the support of the distribution.
The state-of-the-art sensitivity framework~\cite{braverman2016new,bachem2017practical,langberg2010universal} overcomes this challenge by defining the probability distribution with respect to the supremum over all possible $x \in \supp$ of the per-point optimal sampling distribution $p^*(\xx)$:
$$
s_j = \sup_{x \in \supp} p^*(\xx) = \sup_{x \in \supp} \frac{w_{ik}a_k(\xx)}{\sum_{k'} w_{ik'}a_{k'}(\xx)},
$$
and defines $p_k' = s_j/S$, where $S = \sum_{j} s_j$ is the sum of sensitivities. This importance sampling scheme leads to the variance and magnitude of the random variables being bound for \emph{every} input point $\xx \in \supp$:
% fix a single input point $\xx \in \X$ and note that by Jensen's inequality $\E[Y_k^2] = \sum_{k} \frac{w_{ik}^2 a_k^2(\xx)}{p_k} \ge \sum_{k} \frac{w_{ik}^2 a_k^2(\xx)}{p_k} = z(\xx)$, and note that $p_k = \frac{w_{ik}a_k(\xx)}{\sum_{k'} w_{ik'}a_{k'}(\xx)}$ achieves this lower bound

\paragraph{Sampling complexity of existing approaches}
Although the sampling complexity obtained above seems desirable and to be independent of $n = \eta^{\ell}$ at a first glance, note that the sampling complexity grows linearly with the sum of sensitivities, $S$. Unfortunately for the problem of pruning, it can be shown that for all $\edge$,
$
s_k = 1,
$
which implies that $
S = \sum_{j} s_j = n \Rightarrow m \in \Theta(n \, \log(2/\delta) \epsilon^{-2}),
$
% $$
% S = \sum_{j} s_j = n \Rightarrow m \in \Theta( S \, \log(2/\delta) \, \epsilon^{-2}) = \Theta(n \, \log(2/\delta) \epsilon^{-2}),
% $$
leading to a linear sampling complexity.
To see this, note that since we take the supremum of $p^*(\xx)$ over points in the entirety of $\supp$, there could exist a pathological subset of inputs, $\XX_\mathrm{pathological} \subset \supp$, such that for each $x_j \in \XX_\mathrm{pathological}$, we have $a_j(x_j) = \kappa$ for $j = k$ and for some $\kappa >0$, and $a_j(x_j) = 0$ for $j \neq k$, which leads to the numerator and denominator of the sensitivity $s_j$ to be equal. Thus, applying the sensitivity framework to the pruning problem cannot outperform uniform sampling in the general case.

% due to the stringent definition of sensitivity, which requires the computation of a supremum over all $\xx \in \supp$.

% edge cases, don't know distribution, difficult to compute in practice

\paragraph{Our Approach}
The main culprit for the linear sampling complexity of the sensitivity framework is the stringent definition of $\sup_{x \in \supp}$, which does not take into account the probability of drawing a point $x \in \supp$ from $\DD$. As we saw above, there could be a set of pathological inputs in $\supp$ that lead to a sensitivity evaluation of 1, but presumably, this pathological set has measure near-zero, i.e., $\Pr_{x \sim \DD}(x \in \XX_\mathrm{pathological}) \approx 0$, so the probability of drawing a point from $\XX_\mathrm{pathological}$ is extremely low. But, yet the $\sup_{x \in \supp}$ has no consideration of this phenomenon, and naively considers points in the entire distribution (including those in $\XX_\mathrm{pathological}$) when constructing the sampling distribution, which leads to uninformed, uniform sampling in practice. 


In light of our insights, we can ask: rather than taking the supremum over the entirety of $\supp$, can we take a maximum over a small batch of input points $\SS$ instead and bound the variance and magnitude of random variables with high probability (where the randomness is over $x \sim \DD$)? Building upon the work of~\cite{blg2018}, we answer in the affirmative. Namely, introduce the empirical sensitivity of  \emph{empirical sensitivity} as
$$
\hat s_j = \max_{\xx \in \SS} p^*_k(\xx) = \max_{\xx \in \SS} \frac{w_{ik}a_k(\xx)}{\sum_{k'} w_{ik'}a_{k'}(\xx)},
$$
where $\SS$ is a set of $t$ i.i.d. points drawn from $\DD$. We then define $S_\mathrm{emp} = \sum_{j} \hat s_j$ as the sum of the empirical sensitivities and sample from the distribution $q_j = \hat s_j/S_\mathrm{emp}$

By exploiting the inherent stochasticity in the random draw $x \sim \DD$, we establish (see Lemmas~\ref{lem:Ghappens}, \ref{lem:boundM}, and \ref{lem:boundVar}) that with high probability (over the randomness in $\SS$ and $x \sim \DD$)
%in the size of $\SS$, where $t = |\SS| =  \Bigo(\log(1/\delta))$,
$$
\Var(Y_k) \in \Theta(S_\mathrm{emp} \E[Y_k]^2) \quad \text{and} \quad R \in \Theta(S_\mathrm{emp} \E[Y_k]) \Rightarrow m \in \Theta( S_\mathrm{emp} \, \log(2/\delta) \, \epsilon^{-2}).
$$

The sampling complexity we obtain with the sampling distribution defined by empirical sensitivities looks identical to the one for the traditional sensitivity framework with the sole exception of the term $S_\mathrm{emp}$ appearing instead of $S$. This is precisely where the notion of empirical sensitivity shines and enables sublinear sampling complexity. In particular, for $S_\mathrm{emp}$, we have by bounding the maximum over $x \in \SS$ by a sum and rearranging sums: $S_\mathrm{emp} \leq \sum_{\xx \in \SS} \sum_j p^*_k(\xx) = |\SS| = \Bigo(\log(1/\delta))$, which implies that we obtain a sampling complexity that is sublinear in $n$.

The discussion above focused on the case of an arbitrary neuron $i$ for ease of presentation and is based on the work of~\cite{blg2018}. However, to ensure that the maximum variance and magnitude of random variables are bounded in a similar way for each neuron $i \in [\eta^{\ell+1}]$, we extend the work  of~\cite{blg2018} and modify the definition of empirical sensitivity above by taking a $\max_{i \in [\eta^{\ell}]}$ of $p^*_{ik} = \frac{w_{ik} a_k(\xx)}{\sum_{i'} w_{i'k} a_k(\xx)}$ to arrive at our final definition of neuron importance (see Def.~\ref{def:sensitivity}). In light of this change, $S_\mathrm{emp}$ is no longer bounded by $|\SS|$, nevertheless, as our empirical results show, it remains highly sublinear and significantly less than $n$ in practice (see Fig.~\ref{fig:sensitivity}), leading to sublinear sampling complexity. \CB{TODO: Empirical sensitivity figure}

%\CB{Maybe get rid of this?}
% In summary, empirical sensitivity is a data-informed way of constructing an importance sampling scheme that explicitly considers the inherent randomness over the $x \sim \DD$ and focuses on the points that are likely to be drawn in practice when computing the importance assignments to each neuron. In theory, this leads to sublinear sampling complexity (in comparison to linear using the SOTA sensitivity definition), and in practice, leads to a data-informed and efficiently-computable measure of filter importance that can be computed with a small batch of input points $\SS$ and $|\SS|$ forward passes through the network.



% \subsection{An Unbiased Estimator (Property~\ref{prop:unbiased})}
% First we show that Algorithm~\ref{alg:sampling} satisfies property~\ref{prop:unbiased}, i.e., that the resulting estimator is unbiased. To this end, let $a^{\ell}(x)$ denote the activation of layer $\ell$ for an input point $x$ to the network, and $z^{\ell+1}(x)$ denote the pre-activation of layer $\ell + 1$. Note that $a_j^{\ell}(x)$ is the $j$th feature map of layer $\ell$, which is generated by $\WW_j^\ell$. For notational simplicity, we will assume that the layer is linear, i.e., $z^{\ell+1}(x) = W^{\ell+1} a^{\ell}(x)$. The extension to CNNs follows directly as outlined in Appendix~\ref{sec:analysis}. We refer to $\WWHat^\ell$ as being an unbiased estimator of $\WW^\ell$ if the estimator does not incur any bias in the pre-activation $z^{\ell+1}(x)$ in layer $\ell+1$, which depend upon the feature maps $a^\ell(x)$ generated by $\WW^\ell$.
% Note that as a direct consequences of our reweighing scheme (Lines~\ref{lin:start-reweigh}-\ref{lin:end-reweigh}, Alg.~\ref{alg:prune-neurons})our estimator is actually unbiased for any sampling distribution as shown below.
% \begin{lemma}
% The estimator $\WWHat^\ell$ produced by Algorithm~\ref{alg:sampling} gives an unbiased estimator, i.e., $\E_{\WWHat^\ell}[\WW^{\ell+1} a^{\ell}(x)] = \WW^{\ell+1} a^{\ell}(x) = z^{\ell + 1}(x)$.
% \end{lemma}
% \begin{proof}
% We prove the statement for a single output $z = z_i^{\ell+1}(x)$. Note that $z = \sum_j w_{j} a_j$, where $w_{j} = (W^{\ell+1}_j)_{i}$ and $a_j = a_j^{\ell}(x)$. Note that since $W_i^\ell$ gets sampled with probability $p_i$, so does $w_{j}$. Moreover, let $Y_k$, $k \in [m] = [m^\ell]$, be the $k$th sample and note that $Y_k$ takes value $w_{j} a_j$ with probability $p_j$. Then, $\E[Y_k] = \sum_j \frac{w_{j} a_j}{p_j m} \,p_j = \sum_j \frac{1}{m} w_{j} a_j = \frac{z}{m}$. The $i$th entry of the final estimator is then given by $\E[\sum_{k=1}^m Y_k] = z$.
% \end{proof}
% While an unbiased estimator is needed to ensure good performance in expectation, any large deviation can substantially degrade the quality of the estimator in practice.

% \subsection{A Tightly-Concentrated Estimator (Property~\ref{prop:whp})}

==> notes/random.tex <==
Summary of the day (04/24/2019)
\begin{enumerate}
    \item Random sampling with reweighing equally spreads out the contribution to the output. Each sample is an unbiased estimator for the contribution / sample size and removes the particular contribution of that entry
    \begin{enumerate}
        \item Edge sampling with reweighing: weights cancel out and we are left with $$\frac{S a_k}{\max_{x \in \SS} a_k(x)/\dotp{w}{a(x)}}$$.
        The results are still pretty good for (small) fully-connected networks because we are essentially in the regime of matrix sparsification
        \item Neuron sampling with reweighing: sampling distribution is not as informed (because of the max over the columns in definition of sensitivity), so our estimators have high variance leading to worse performance than deterministic even on fully-connected networks
        \item Neuron sampling without reweighing: essentially the same empirical performance as deterministic, because we expect to sample the high-sensitivity neurons anyway
        \item The main problem with reweighing for \textbf{trained networks} seems to be that training leads to important paths/neurons such that reweighing (and in effect equally distributing the output) destroys these path connections. Training may also lead to interlayer dependencies between the outputs of the neurons (which we do not capture with local sensitivity)
        \item Optimized network -> Pruning -> Retraining: the problem with reweighing in this case is that after the initial training, the weights are close to a local minimum and sensitivity captures the importance of the weights for that local minimum. But now, if we reweigh the weights, we essentially keep the important weights, BUT throw away their values (which define the local minimum), leading to an initialization that is far away from local minima in the retraining phase. Long story short: reweighing pushes the weights (that were initially close to a local minimum) further away from the local minimum!!!!!!!
    \end{enumerate}
    \item Random initialization -> Pruning -> Training: reweighing does help in this scenario, possibly due to the fact that by spreading out the contribution of the output, the Lipschitz constant of the network is lowered, leading to a smoother optimization landscape (see Madry's paper)
\end{enumerate}

Story for the paper:
\begin{enumerate}
    \item We do random sampling of neurons on randomly initialized networks and then train 
    \item First, sensitivity captures the neurons that are important after the random initialization and then we use sensitivity to prune away unimportant neurons
    \item During the sampling process, we reweigh the sampled neurons and debias them. This helps lowering the Lipschitz constant, thus creating a smoother optimization landscape. 
    \item We can then train the smaller architectures and obtain much better results than directly initializing the network
    \item What's the differene to just using a small network in the first place: Using a small network makes it harder to train (cite papers about that). It seems that random initialization is helpful, but only for large networks since you need a lot of randomness to get lucky. Then training usually extracts out the "lucky" neurons and makes them important. We extract them right away with sensitivity-based sampling. 
    \item Two view points: "Efficient architecture search" or "smart random initialization" also mention lottery ticket hypothesis, who takes a similar stance 
    \item Why the local sensitivity approach does not hurt us: There is no direct interdependency between layers besides the data. We do capture the dependency on the data, but unlike in the case of training first, there are no important paths that originated from the training that we could potentially destroy.
    \item Proofs or analytical results. two ideas
    \begin{enumerate}
        \item We show that our approach yields a lower Lipschitz constant than directly randomly initializing a small network. This supports the view point of "data-informed initialization".
        \item We show that sensitivity does not change much during training, which implies that we can provably prune the untrained networks just as we could have pruned the trained network. This supports the view point of "efficient architecture search" 
    \end{enumerate}
    \item For the experiments: we won't need to do experiments with training first, we simply do experiments with random init -> pruning -> training. 
\end{enumerate}

Interesting things to prove:
\begin{enumerate}
    \item Reweighing helps initialization: Random initialization -> pruning -> reweighing is more favorable for training than training from random initialization of a network \textbf{of the same size of the pruned network}
    \item Optimal loss after training compressed network $\epsilon$-approximates optimal loss of original network after training: Optimal solution to the network obtained by \textit{Random initialization -> pruning -> reweighing} achieves a similar loss as does the optimal solution to the randomly initialized then trained network
\end{enumerate}
